What's Your Value of Travel Time? Collecting Traveler-Centered Mobility Data via Crowdsourcing

Mobility and transport, by their nature, involve crowds and require the coordination of multiple stakeholders - such as policy-makers, planners, transport operators, and the travelers themselves. However, traditional approaches have been focused on time savings, proposing to users solutions that include the shortest or fastest paths. We argue that this approach towards travel time value is not centered on a traveler's perspective. To date, very few works have mined data from crowds of travelers to test the efficacy and efficiency of novel mobility paradigms. In this paper, we build upon a different paradigm of worthwhile time in which travelers can use their travel time for other activities; we present a new dataset, which contains data about travelers and their journeys, collected from a dedicated mobile application. Each trip contains multi-faceted information: from the transport mode, through its evaluation, to the positive and negative experience factors. To showcase this new dataset's potential, we also present a use case, which compares corresponding trip legs with different transport modes, studying experience factors that negatively impact users using cycling and public transport as alternatives to cars. We conclude by discussing other application domains and research opportunities enabled by the dataset.

==> tables/all_experience_factor.tex <==
% Right alignment for p{length} box in tabular
% See:
%   https://tex.stackexchange.com/a/338010/25748
%\begin{tabular}{@{}lrlrlr@{}}
\begin{tabular}%
  {@{}%
   >{\raggedright\arraybackslash}p{4cm}%
   >{\raggedleft\arraybackslash}p{1cm}%
   >{\raggedright\arraybackslash}p{4cm}%
   >{\raggedleft\arraybackslash}p{1cm}%
   >{\raggedright\arraybackslash}p{4cm}%
   >{\raggedleft\arraybackslash}p{1cm}%
   @{}%
  }
\toprule
  \multicolumn{2}{c}{\textbf{Cycling and micromobility}}
& \multicolumn{2}{c}{\textbf{Public transport (short distance)}}
& \multicolumn{2}{c}{\textbf{Public transport (long distance)}} \\
  \textbf{Factor}                  & \textbf{\#} 
& \textbf{Factor}                  & \textbf{\#}
& \textbf{Factor}                  & \textbf{\#} \\
\cmidrule{1-2}\cmidrule{3-4}\cmidrule{5-6}
Cars other vehicles                & $1,751$ & Privacy                        & $500$ & Internet connectivity          & $53$ \\
Air Quality                        & $1,277$ & Crowdedness seating            & $499$ & Privacy                        & $49$ \\
Road path availability and safety  & $1,219$ & Other people                   & $463$ & Seating quality personal space & $44$ \\
Noise level                        & $1,097$ & Seating quality personal space & $445$ & Reliability of travel time     & $43$ \\
Road path quality                  &   $969$ & Noise level                    & $437$ & Noise level                    & $36$ \\
Traffic signals crossings          &   $854$ & Internet connectivity          & $418$ & Other people                   & $35$ \\
Crowding congestion                &   $837$ & Charging opportunity           & $406$ & Vehicle ride smoothness        & $34$ \\
Today's weather                    &   $591$ & Air quality                    & $349$ & Today's weather                & $34$ \\
Simplicity difficulty of the route &   $417$ & Scenery                        & $309$ & Crowdedness seating            & $33$ \\
Facilities shower lockers          &   $371$ & Reliability of travel time     & $290$ & Food drink available           & $31$
\\ \bottomrule
\end{tabular}

==> tables/case_study.tex <==
\begin{tabular}{@{}lp{2.8cm}rrr@{}}
\toprule
\textbf{Step} & \textbf{Step description} & \textbf{Trips} & \textbf{Legs} & \textbf{Users} \\ \midrule
1          & All trips, legs, users
                                          &       $64,098$ &     $158,897$ &        $3,269$ \\
2          & Users that have performed at least one trip leg by car
                                          &       $21,764$ &      $62,227$ &        $2,083$ \\
3          & Users that have selected at least one preferred alternative transport mode
                                          &       $51,973$ &     $132,259$ &        $1,771$ \\
4          & Users that have performed at least one trip leg by car and by alternative transport modes
                                          &       $20,032$ &      $27,921$ &        $1,376$ \\ \bottomrule
\end{tabular}

==> tables/legs.tex <==
\begin{tabular}{@{}p{4.5cm}p{12.5cm}@{}}
\toprule
\textbf{Field}
          & \textbf{Description and admissible values} \\ \midrule
\texttt{legid}
          & Leg identifier, a string in the format \texttt{\#\{n1\}:\{n2\}} where \texttt{n1} and \texttt{n2} are two numbers. \\
\texttt{class}
          & Leg type, either \texttt{Leg} or \texttt{WaitingEvent}. \\
\texttt{userid}
          & User identifier. \\
\texttt{tripid}
          & Trip identifier. \\
\texttt{motid}
          & Mode of transport identifier, an integer number. \\
\texttt{start\_date}
          & Leg start date, formatted as \texttt{\%Y-\%m-\%d \%H:\%M:\%S.\%f}. \\
\texttt{end\_date}
          & Leg end date, formatted as \texttt{\%Y-\%m-\%d \%H:\%M:\%S.\%f}. \\
\texttt{true\_distance}
          & Leg distance in meters. \\
\texttt{leg\_distance}
          & Leg distance in meters. \\
\texttt{leg\_duration}
          & Leg duration in seconds. \\
\texttt{worthwhileness\_rating}
          & Worthwhileness rating, $-1$ if not set. \\
\texttt{transport\_category}
          & Transport category. \\
\texttt{campaign}
          & Data collection campaign. \\
\texttt{weekday}
          & Day of the week when the leg was performed. \\
\texttt{weekday\_class}
          & Classification of the day, either \texttt{Working\_day} or \texttt{Weekend}. \\
\bottomrule
\end{tabular}

==> tables/legs_coordinates.tex <==
%\ra{1.2}
\begin{tabular}{@{}p{3.0cm}p{14.0cm}@{}}
%\hline
\toprule
\textbf{Field}          & \textbf{Description and admissible values}                                                       \\ \hline                                                       
\texttt{leg\_id}                              & The identifier of the leg in the format \#n1:n2, with n1 and n2 being two integer numbers.                                                                                                             \\ 
\texttt{start\_lat}                           & a real number with 3 decimals. The latitude of the starting point of the leg.                                                                                                                          \\ 
\texttt{start\_lon}                           & a real number with 3 decimals. The longitude of the starting point of the leg.                                                                                                                         \\ 
\texttt{end\_lat}                             & a real number with 3 decimals. The latitude of the ending point of the leg.                                                                                                                            \\ 
\texttt{end\_lon}                             & a real number with 3 decimals. The longitude of the ending point of the leg.                                                                                                                           \\ 
\texttt{start\_name}                          & The inferred name of the city where the starting point of the leg is located. This field is obtained in the preprocessing by integrating the leg coordinates with OECD data.                           \\ 
\texttt{start\_country}                       & The ISO 3166 Alpha-3 code of the inferred country where the starting point of the leg is located. This field is obtained in the preprocessing by integrating the leg coordinates with OECD data1b.     \\ 
\texttt{start\_class}                         & Possible values are: urban, sub-urban, or rural. The classification of the starting point of the leg. This field is obtained in the preprocessing by integrating the leg coordinates with OECD data1c. \\ 
\texttt{end\_name}                            & The inferred name of the city where the ending point of the leg is located. This field is obtained in the preprocessing by integrating the leg coordinates with OECD data.                             \\ 
\texttt{end\_country}                         & The ISO 3166 Alpha-3 code of the inferred country where the ending point of the leg is located. This field is obtained in the preprocessing by integrating the leg coordinates with OECD data1b.       \\ 
\texttt{end\_class}                           & Possible values are: urban, sub-urban, or rural. The classification of the ending point of the leg. This field is obtained in the preprocessing by integrating the leg coordinates with OECD data1c.   \\ \bottomrule
\end{tabular}

==> tables/selected_experience_factors.tex <==
% Right alignment for p{length} box in tabular
% See:
%   https://tex.stackexchange.com/a/338010/25748
%\begin{tabular}{@{}lrlrlr@{}}
\begin{tabular}%
  {@{}%
   >{\raggedright\arraybackslash}p{4cm}%
   >{\raggedleft\arraybackslash}p{1cm}%
   >{\raggedright\arraybackslash}p{4cm}%
   >{\raggedleft\arraybackslash}p{1cm}%
   >{\raggedright\arraybackslash}p{4cm}%
   >{\raggedleft\arraybackslash}p{1cm}%
   @{}%
  }
\toprule
  \multicolumn{2}{c}{\textbf{Cycling and micromobility}}
& \multicolumn{2}{c}{\textbf{Public transport (short distance)}}
& \multicolumn{2}{c}{\textbf{Public transport (long distance)}} \\
  \textbf{Factor}                  & \textbf{\#} 
& \textbf{Factor}                  & \textbf{\#}
& \textbf{Factor}                  & \textbf{\#} \\
\cmidrule{1-2}\cmidrule{3-4}\cmidrule{5-6}
Road path availability and safety  & $315$ & Privacy                        & $133$ & Today's weather             & $2$ \\
Road path quality                  & $307$ & Other people                   & $111$ & Reliability of travel time  & $2$ \\
Cars other vehicles                & $267$ & Air quality                    & $103$ & Vehicle ride smoothness     & $1$ \\
Air quality                        & $173$ & Noise level                    & $100$ & Ability to do what I wanted & $1$ \\
Noise level                        & $132$ & Crowdedness seating            &   $99$ & Privacy                     & $1$ \\
Road path directness               & $131$ & Seating quality personal space &   $99$ & Other people                & $1$ \\
Today's weather                    & $123$ & Today's weather                &   $84$ & Cleanliness                 & $1$ \\
Traffic signals crossings          & $122$ & Internet connectivity          &   $77$ &                             &     \\
Crowding congestion                & $111$ & Charging opportunity           &   $76$ &                             &     \\
Lighting visibility                &  $88$ & Scenery                        &   $67$ &                             &
\\ \bottomrule
\end{tabular}


==> tables/trips.tex <==
\begin{tabular}{@{}p{4.5cm}p{12.5cm}@{}}
\toprule
\textbf{Field}
                                  & \textbf{Description and admissible values} \\ \hline
\texttt{tripid}
                                  & Trip identifier, a string in the format \texttt{\#\{n1\}:\{n2\}} where \texttt{n1} and \texttt{n2} are two numbers. \\
\texttt{userid}
                                  & User identifier. \\
\texttt{start\_date}
                                  & Trip start date, formatted as '\%Y-\%m-\%d \%H:\%M:\%S.\%f'. \\
\texttt{end\_date}
                                  & Trip end date, formatted as '\%Y-\%m-\%d \%H:\%M:\%S.\%f'. \\
\texttt{average\_speed}
                                  & Average speed during trip in km/h. \\
\texttt{max\_speed}
                                  & Max speed during trip. \\
\texttt{distance}
                                  & Leg distance in meters. \\
\texttt{duration}
                                  & Leg duration in seconds. \\
\texttt{mood\_rating}
                                  & Evaluation of trip mood on a scale from 1 to 5. \\
\texttt{did\_you\_have\_to\_arrive}
                                  & Answer to the question \emph{``Did you have to arrive on time''}, a boolean value. \\
\texttt{how\_often}
                                  & Answer to the question \emph{``How often do you make this trip?''}, possible values are integers from \texttt{0} to \texttt{3}. \texttt{-1} means that the question was not answered. \\
\texttt{use\_trip\_more\_for}
                                  & Answer to the question \emph{``How often do you make this trip?''}, possible values are integers from \texttt{0} to \texttt{3}. \texttt{-1} means that the question was not answered. \\
\texttt{manual\_start}
                                  & Answer to the question \emph{``Has the trip recording been started manually?''}, a boolean value. \\
\texttt{manual\_end}
                                  & Answer to the question \emph{``Has the trip recording been ended manually?''}, a boolean value. \\
\texttt{validation\_date}
                                  & Trip validation date, formatted as '\%Y-\%m-\%d \%H:\%M:\%S.\%f'. \\
\texttt{os}
                                  & Operating system of the phone, can be \texttt{iOS} or \texttt{Android}, a string.  \\
\texttt{os\_version}
                                  & Operating system version, a string. \\
\texttt{model}
                                  & Model of the phone, a string. \\  
\bottomrule
\end{tabular}

==> tables/user_details.tex <==
\begin{tabular}{@{}p{3.5cm}p{12.5cm}@{}}
  \toprule
  \textbf{Field}
                                      & \textbf{Description and admissible values} \\ \hline
  \textbf{\texttt{user\_id}}${}^{*}$
                                      & User identifier, a string of 29 charaters. \\
  \textbf{\texttt{registration\_timestamp}}${}^{*}$
                                      & Trip start date, formatted as \texttt{\%Y-\%m-\%d \%H:\%M:\%S.\%f}. \\
  \textbf{\texttt{gender}}${}^{*}$
                                      & Gender of the user. Three values are possible: \texttt{Other}, \texttt{Male}, \texttt{Female}. \\
  \textbf{\texttt{age}}${}^{*}$
                                      & User's age in a range. Possible values are: \texttt{16-19}, \texttt{20-24}, \texttt{25-29}, \texttt{30-39}, \texttt{40-49}, \texttt{50-64}, \texttt{65-74}, \texttt{75+}.  \\
  \texttt{language}
                                      & Language used for the \emph{Woorti} app expressed as a 3-letter ISO 639-2/B code. \\
  \texttt{city}
                                      & User's city of residence. \\
  \texttt{country}
                                      & User's country of residence expressed in ISO 3166-1 alpha-3 code. \\
  \texttt{education\_level}
                                      & User's education, possible values are: \texttt{Basic (up to 10th grade)}, \texttt{High School (12th grade)}, and \texttt{University} \\
  \texttt{marital\_status}
                                      & User's marital status, possible values are: \texttt{Single}, \texttt{Registered relationship}, \texttt{Married}, \texttt{Divorced}, \texttt{Widowed}. \\
  \texttt{number\_of\_people}
                                      & Number of people in the household, it can be a number from $1$ to $4$ or $5+$. \\
  \texttt{labour\_status}
                                      & Users's labour status. Possible values are: \texttt{Student}, \texttt{Employed full-time}, \texttt{Employed part-time}, \texttt{Pensioner}, \texttt{Unemployed}. \\
  \texttt{years\_of\_residence}
                                      & Years of residence in the household and possible values are: \texttt{Less than 1}, \texttt{1 to 5}, \texttt{More than 5}. \\
  \bottomrule
\end{tabular}

==> tables/weather_legs.tex <==
\begin{tabular}{@{}p{5.0cm}p{12.0cm}@{}}
\toprule
\textbf{Field}
          & \textbf{Description and admissible values} \\ \midrule
\texttt{weatherid}
          & Weather identifier, a string of 24 characters. \\
\texttt{legid}
          & Leg identifier. \\
\texttt{request\_date}
          & Weather request timestamp, formatted as '\%Y-\%m-\%d \%H:\%M:\%S.\%f'. \\
\texttt{centroid\_x}
          & Longitude of the centroid of the leg. \\
\texttt{centroid\_y}
          & Latitude of the centroid of the leg. \\
\texttt{country}
          & Country the leg is located in. \\
\texttt{weather\_scenario}
          & Classification of weather scenarios. \\
\texttt{apparent\_temperature}
          & Apparent temperature, computed using Steadman's equation. \\
\texttt{net\_radiation}
          & Net radiation received by the terrain in the location of the centroid. \\
\texttt{temperature\_category}
          & Categorization based on apparent temperature. \\
\texttt{temperature\_description}
          & Description of the temperature based on apparent temperature. \\
\texttt{cloud\_category}
          & Categorization based on cloud cover. \\
\texttt{cloud\_main}
          & Description based on cloud cover. \\
\texttt{precipitation\_category}
          & Categorization based on precipitation level. \\
\texttt{precipitation\_main}
          & Description based on precipitation level. \\
\texttt{wind\_beaufort\_number}
          & Categorization using Beaufort's number, based on wind speed. \\
\texttt{wind\_category}
          & Categorization based on wind speed. \\
\texttt{wind\_description}
          & Description based on wind speed. \\
\bottomrule
\end{tabular}

